On the Limitation and Experience Replay for GNNs in Continual Learning

Continual learning seeks to empower models to progressively acquire information from a sequence of tasks. This approach is crucial for many real-world systems, which are dynamic and evolve over time. Recent research has witnessed a surge in the exploration of Graph Neural Networks (GNN) in Node-wise Graph Continual Learning (NGCL), a practical yet challenging paradigm involving the continual training of a GNN on node-related tasks. Despite recent advancements in continual learning strategies for GNNs in NGCL, a thorough theoretical understanding, especially regarding its learnability, is lacking. Learnability concerns the existence of a learning algorithm that can produce a good candidate model from the hypothesis/weight space, which is crucial for model selection in NGCL development. This paper introduces the first theoretical exploration of the learnability of GNN in NGCL, revealing that learnability is heavily influenced by structural shifts due to the interconnected nature of graph data. Specifically, GNNs may not be viable for NGCL under significant structural changes, emphasizing the need to manage structural shifts. To mitigate the impact of structural shifts, we propose a novel experience replay method termed Structure-Evolution-Aware Experience Replay (SEA-ER). SEA-ER features an innovative experience selection strategy that capitalizes on the topological awareness of GNNs, alongside a unique replay strategy that employs structural alignment to effectively counter catastrophic forgetting and diminish the impact of structural shifts on GNNs in NGCL. Our extensive experiments validate our theoretical insights and the effectiveness of SEA-ER.

==> ICLR_format/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tex/ablation_study.tex <==
\section{Ablation Study}\label{sec:ablation_study}


\subsection{CMD effective}
In this experiment, we want to demonstrate that CMD is indeed an effective indicator for generalization performance of GNN, and use it as a regularizer can indeed 1) bring the learnt representation closer and 2) improve the performance of GNN

\subsection{Distribution Distance and Replaying Method}
In this experiment, we want to demonstrate that our replaying set selection strategy provide the best representative samples in term of distribution distance for underlying data population.

\subsection{Standard Ablation Study}
In this experiment, we want to demonstrate the effectiveness of the components of our framework one by one.


==> tex/analysis.tex <==
\subsection{Theoretical Analysis}\label{sec:theory}
In this section, we delve into the theoretical underpinnings of our proposed method by introducing the concept of distortion rate, which aids in characterizing the topological awareness of GNNs.

A GNN is said to have a distortion rate $\alpha$ if there exists a constant $r > 0$ such that for all $u,v \in \mathcal{V}$, the following inequalities hold: $\forall u,v \in \mathcal{V},  r d_{\mathrm{spd}}(u,v) \leq d(h_u,h_v)\leq \alpha r d_{\mathrm{spd}}(u,v).$  The distortion rate quantifies the ratio of distances in the embedding space to those in the original graph space. A low distortion rate, close to 1, signifies that the embedding effectively preserves the structural information from the original graph. This measure allows us to assess the topological awareness of GNNs and forms the basis for our theoretical analysis of the experience selection strategy in relation to the underlying graph topology.

\begin{proposition}\label{thm:performance_guarantee}
Given a collection task $\task_1,...,\task_m$ and their associated vertex set $\vertexSet_1,...,\vertexSet_m$. Let $\experienceBuffer_m = \{P_1,...,P_{m-1}\}$ be the experience buffer where each $P_i \in \experienceBuffer_m$ has the same cardinality and cover all classes in $\task_i$. 
Let $\gnnModel$ be the GNN model with distortion rate $\alpha$. Assuming the loss function $\loss$ is bounded, continuous and smooth, we have that,
    % $$R^{\loss}(\vertexSet_i \backslash P_i) \leq R^{\loss}(P_i) + \mathcal{O} (\alpha  D_s(\vertexSet_i \backslash P_i,P_i)),$$
    $$ R_{\jointDistCondVertSet{v}{\vertexSet_i \backslash P_i}}^{\loss}(f) \leq R_{\jointDistCondVertSet{v}{ P_i}}^{\loss}(f) + \mathcal{O} (\alpha  D_s(\vertexSet_i \backslash P_i,P_i)),$$
where 
$$
  D_s(\vertexSet_i \backslash P_i,P_i) = \max_{u \in \vertexSet_i \backslash P_i}\min_{v \in P_i} d_{\mathrm{spd}}(v, u).
$$
\end{proposition}

The proof for Propostion~\ref{thm:performance_guarantee} can be found in Appendix~\ref{appendix:structural_relation}. This proposition illuminates that catastrophic forgetting in the model, as measured by its ability to retain performance on past data, is bounded by the training loss on the experience buffer and is further influenced by a combination of factors involving the distortion rate of the model and the structural distance within the experience buffer. This underscores the critical role of graph structure when selecting a suitable experience buffer, as the structural distance substantially impacts the performance bound. Consequently, Proposition~\ref{thm:performance_guarantee} validates the optimization objective, Eq.~\ref{eq:experience_buff}, for selecting an experience buffer and provides a performance guarantee for our proposed experience selection strategy.


% \begin{definition}[distortion rate]\label{def:distortion}
%     Given two metric spaces $(\mathcal{Q},d)$ and $(\mathcal{Q'},d')$ and  
%  	a mapping $\gamma: \mathcal{Q} \mapsto \mathcal{Q'}$, $\gamma$ is said to have a distortion $\alpha \geq 1$, if there exists a constant $r > 0$ such that $\forall u,v \in \mathcal{E}$, $ r d(u,v) \leq d'(\gamma(u),\gamma(v))\leq \alpha r d(u,v)$.
% \end{definition}

% The distortion rate captures the ratio of the distance in the embedding space to that in the original graph space. A low distortion rate (close to 1) indicates that the embedding preserves the corresponding structural information from the original space. We use distortion rate to characterize the topological awareness of GNNs, which allows us to theoretically analyze our experience selection strategy with respect to the underlying topology.  

==> tex/challenge.tex <==
\subsection{Unique Challenges in NGIL}\label{sec:bias}

{\bf Structural Dependency.} The structural dependency of the graph structure among different tasks poses a significant challenge in the inductive NGIL setting. As the system is tasked with learning from a set of node classification tasks that arrive sequentially, it must continuously acquire new knowledge while retaining previously obtained knowledge. However, the appearance of new vertices from new tasks can expand the previous graph structure and alter the dependencies among vertices in previous tasks. This can lead to a fundamental change in the information learned by GNNs, as they rely on neighborhood aggregation to learn representations for each vertex. This is further illustrated in Fig.~\ref{fig:data_dependency}, where the 2-hop ego graph of a red vertex $v$ has changed significantly with the addition of new vertices from a new task. On the other hand, in a transductive setting, the ego graph of vertices stays the same. In other words, structural dependency can induce a distributional shift in the information learned from previous tasks in the inductive setting and needs to be addressed in the experience replay method.


\vspace{1mm}
\noindent{\bf Structural Bias.} In addition to considering the structural dependency of the graph, it is also important to address the issue of structural bias of GNNs in NGIL, particularly, for selecting the experience buffer. Structural bias refers to the tendency of GNNs to exhibit unfair behaviour towards different structural subgroups (subgroups defined by a graph structure such as distance) within the data~\cite{subgroup,cmd_gnn}. This can result in a large variance in the performance of GNNs when trained on different subsets of vertices, particularly when the number of samples is small, as is the case with experience replay. To avoid this, it is important to carefully select a representative sample from the past for experience replay, taking into account the structural properties of the data and the predictive power of GNNs. 

 % An illustration of this can be seen in Fig.\ref{fig:random_training_set_cora}, where representative GNN models, GCN~\cite{gcn}, GAT~\cite{gat}  and GraphSage~\cite{sage}, are trained on the commonly used CORA dataset~\cite{common_data} for a node classification problem. The figure demonstrates a significant variance in the generalization of the models with different subsets, which can have a significant impact on the performance of the experience replay method if the experience buffer is not selected carefully. 

\begin{figure*}[!t]
\vspace{-1.3cm}
\centering
\includegraphics[width=0.8\textwidth{figures/framework/diff_constant_evovling.drawio.png}
\caption{An illustration of the difference between transductive and inductive NGIL. $\task_1$ and $\task_2$ are two consecutive tasks. In the transductive setting, the 2-hop ego graph of the vertex with a red circle would remain the same, while in the inductive setting, the graph may change as new tasks are introduced and the overall graph structure evolves. 
}
\label{fig:data_dependency}
\end{figure*}

% \begin{figure}[!t]
% % \vspace{-1.3cm}
% \centering
% \includegraphics[width=0.48\textwidth]{figures/framework/diff_constant_evovling.drawio_half.png}
% \caption{An Illustration of Structural Dependency Issue in the Inductive NIGL and the Difference from the Transductive Setting.  
% }
% \label{fig:data_dependency}
% \end{figure}


% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/experiment/rts_cora.pdf}
% % \includegraphics[width=0.235\textwidth]{figures/experiment/rts_citeseer.pdf}
% \caption{An Illustration of Structural Bias of GNNs. Performance of GCN,  
% GraphSAGE, and GAT
% on Cora dataset with different randomly selected training sets (5 vertices from each classes) and test set (the rest of labelled vertice). 
% }
% \label{fig:random_training_set_cora}
% \end{figure}



==> tex/preliminary.tex <==

\section{Preliminary and Problem Formulation}\label{sec:problem_formulation}
In this section, we present the preliminary and formulation of the inductive NGIL problem. We use bold letters to denote random variables, while the corresponding realizations are represented with thin letters.


We assume the existence of a stream of training tasks $\task_1, \task_2,..., \task_m$, characterized by observed vertex batches $\vertexSet_1,\vertexSet_2,...,\vertexSet_m$. Each vertex $v$ is associated with a node feature $x_v$ and a target label $y_v$. The observed graph structure at training task $\task_i$ is induced by the accumulative vertices and given by $\graphStruct_{\task_i} = \graphStruct[\bigcup_{j=1}^i \vertexSet_j]$. In this setting, the graph structure is evolving as the learning progresses through different training tasks. Fig.~\ref{fig:ngil} provides a graphical illustration.  

To accommodate the nature of node-level learning tasks, in which the information used for inference is aggregated within the k-hop neighborhood of a node, we adopt a local view in the learning problem formulation. We define $\neighbor{k}(v)$ as the k-hop neighborhood of vertex $v$, and the nodes in $\neighbor{k}(v)$ form an ego-graph $\ego{v}$, which consists of a (local) node feature matrix $X_v = \{x_u |u \in \neighbor{k}(v)\}$ and a (local) adjacency matrix $A_v = \{a_{uw}|u,w \in \neighbor{k}(v)\}$. We use $\rand{\ego{v}}$ as a random variable of the ego-graph for the target vertex $v$, whose realization is $\ego{v} = (A_v,X_v)$.  %Furthermore, we denote 
Let $\ego{\vertexSet} = \{\ego{v} |v \in \vertexSet \}$ denote the set of ego graphs associated with vertex set $\vertexSet$. Under this formulation, the ego-graph $\ego{v}$ can be viewed as the Markov blanket (containing all necessary information for the prediction problem) for the root vertex $v$. Therefore, we can see the prediction problem associated with data $\{(\ego{v},y_v)\}_{v \in \vertexSet_i}$ from training session $\task_i$ as drawn from an empirical joint distribution $\prob(\mathbf{y_{v}},\mathbf{G}_{v}|\vertexSet_i)$.


Let $\hypothesis$ denote the hypothesis space and $f \in \hypothesis$ be a classifier with $\hat{y}_v = f (G_v)$ and $\loss(.,.) \mapsto \R$ be a given loss function. We use $R_{\jointDistCondVertSet{v}{\vertexSet}}^{\loss}(f)$ to denote the generalization risk of the classifier $f$ with respect to $\loss$ and $\jointDistCondVertSet{v}{\vertexSet}$, and it is defined as follows:
 \begin{equation}\label{eq:gen_risk}
     R_{\jointDistCondVertSet{v}{\vertexSet}}^{\loss}(f) = \expect_{\jointDistCondVertSet{v}{\vertexSet}}[\loss(f(\ego{v}),y_v)].
 \end{equation}


{\bf Catastrophic Forgetting Risk.}
With the formulation above, the catastrophic forgetting risk ($\cataForget$) of a classifier $f$ after being trained on $\task_m$ can be characterized by the retention of performance on previous vertices, given by: 
\begin{equation}\label{eq:cf}
\begin{split}
      \cataForget(f) & := R_{\jointDistCondVertSet{v}{\vertexSet_1,...,\vertexSet_{m-1}}}^{\loss}(f)
\end{split}
\end{equation}
which translates to the retention of performance of the classifier $f$ from $\task_m$ on the previous tasks $\task_1,...,\task_{m-1}$.


% \section{Preliminaries and Problem Formulation }\label{sec:preliminary}
% In this section, we introduce the formulation of the inductive NGIL problem, GNNs, and experience replay framework.

% The inductive NGIL problem involves a collection of $m$ tasks  $\task = \{ \task_1, \task_2, ..., \task_m \}$ that are encountered sequentially, where each $\task_i \in \task$ is a node classification task. Formally, a node classification task is defined as:

% \begin{definition}
% For each node classification task $\task_i$, there is a training node set $\vertexSet^{\mathrm{train}}_i$ and a testing node set $\vertexSet^{\mathrm{test}}_i$. The goal of the learning task is to learn a task-specific classifier $f_{\task_i}$ from $\vertexSet^{\mathrm{train}}_i$ that correctly classifies each vertex $v \in \vertexSet^{\mathrm{test}}_i$ into its correct label $y_v \in \mathcal{Y}_i$, where $\mathcal{Y}_i = \{y_1^i, y_2^i, ..., y_k^i\}$ is the label set and $k$ is the number of classes in $\task_i$.
% \end{definition}

% We consider an inductive setting where the task collection $\task$ is drawn from an unknown undirected graph $\graphStruct$. Let $\vertexSet_i$ denote the set of vertices associated with $\task_i$. Then the observed graph structure at task $\task_i$ is induced by the cumulative vertices from all encountered tasks before, and is given by:
% $\graphStruct_{\task_i} = \graphStruct[\bigcup_{j=1}^i \vertexSet_j].$
% In this setting, the graph structure evolves as the learning progresses through different training tasks. We have:
% $\mathcal{G}_{\taskSet_i} \subset \mathcal{G}_{\taskSet_{i+1}}, \forall i \in 1,..., m-1.$

% Fig.~\ref{fig:data_grow} provides a graphical illustration. This setting is significantly different from the transductive setting which assumes the complete graph structure is known throughout each task. We further discuss how the indutive setting is different in the next section. 

% \begin{figure}[!t]
% \centering
% \vspace{-0.6cm}
% \includegraphics[width=0.48\textwidth]{figures/framework/two-stage.drawio.png}
% \caption{An Illustration of inductive NGIL. For each new task, the graph structure evolves and expands. The different coloured vertexes within each task represent the different classes/labels within the classification task. The vertexes highlighted in red are the vertexes whose neighbourhoods are altered by the expansion process. The overlapped region indicates that a vertex can belong to more than one task.
% }
% \vspace{-0.1cm}
% \label{fig:data_grow}
% \end{figure}


% \subsection{Graph Neural Network}
% GNNs are a class of neural networks that operate on graph-structured data. They adopt a neighbourhood aggregation scheme, where the representation of a node is updated iteratively by aggregating representations of its neighbours. After $k$ iterations of aggregation, a node's representation captures the structural information within its k-hop neighborhood in the graph. Formally, the k-th layer of a GNN can be written as follows:

% \begin{equation}
%     h_{u}^{(k)} = \mathrm{Update}^{(k)}(\mathrm{Aggregate}^{(k)}({h_v^{(k-1)}, \forall v \in \mathcal{N}(u) \cup \{u\} })),
% \end{equation}

% \noindent where $h_u^{(k)}$ is the representation vector of node $u$ at the k-th layer, $h_u^{(0)}$ is initialized to be the node feature of vertex $x_u$, and $\mathcal{N}(u)$ is the set of nodes adjacent to $u$. Different GNNs are compositions of these aggregation and update layers with different designs. Such a neighborhood scheme allows GNNs to capture structural information of a given vertex. In node classification tasks, GNNs are used as an embedding function (to capture structural information) along with some task-specific prediction functions to form the task-specific classifier. More formally, we refer to $\gnnModel$ as a given GNN model and $f_{\task_i}$ as the task-specific classifier for task $\task_i$. Then the predicted classification of vertex $v$ from task $\task_i$ is given by $\hat{y_v} = f_{\task_i} (\gnnModel(v)) $.



% \subsection{Experience Replay Framework}
% Experience replay is a method inspired by the Complementary Learning Systems (CLS) theory, which suggests that human learning involves a virtual experience system that replays stored memory to continually reinforce tasks that have been recently performed~\cite{replay_psy1,replay_psy2}. The idea of experience replay is to select a small subset of representative data samples from the past and to replay them in each new learning task to consolidate past knowledge. Experience replay methods involve two main components: 1) selecting replay samples from the past to be stored in the experience buffer, and 2) deciding how the experience buffer is replayed (trained) with the new task.

% Given a loss function $\loss$, let $\loss(v)$ denote the loss for vertex $v$. $\experienceBuffer_i = \{P_1,...,P_{i-1}\}$ denotes the experience buffer accumulated before task $\task_i$ and $P_j \in \experienceBuffer_i$ is the replay samples selected from task $\task_j$ based on certain strategy. Then, a standard experience replay framework amounts to the following learning objective:
% \begin{equation}\label{eq:common_learning}
%    \loss = \frac{1}{|\vertexSet^{\mathrm{train}}_i|} \sum_{v \in \vertexSet^{\mathrm{train}}_i} \loss(v) + \sum_{P_j \in \experienceBuffer_i}\frac{1}{|P_j|}\sum_{v \in P_j}\loss(v),
% \end{equation}
% where $\vertexSet^{\mathrm{train}}_i$ is the training set for task $\task_i$. 


